GROUNDHOG: Grounding Large Language Models to Holistic Segmentation

Most multimodal large language models (MLLMs) learn language-to-object grounding through causal language modeling where grounded objects are captured by bounding boxes as sequences of location tokens. This paradigm lacks pixel-level representations that are important for fine-grained visual understanding and diagnosis. In this work, we introduce GROUNDHOG, an MLLM developed by grounding Large Language Models to holistic segmentation. GROUNDHOG incorporates a masked feature extractor and converts extracted features into visual entity tokens for the MLLM backbone, which then connects groundable phrases to unified grounding masks by retrieving and merging the entity masks. To train GROUNDHOG, we carefully curated M3G2, a grounded visual instruction tuning dataset with Multi-Modal Multi-Grained Grounding, by harvesting a collection of segmentation-grounded datasets with rich annotations. Our experimental results show that GROUNDHOG achieves superior performance on various language grounding tasks without task-specific fine-tuning, and significantly reduces object hallucination. GROUNDHOG also demonstrates better grounding towards complex forms of visual input and provides easy-to-understand diagnosis in failure cases.

==> sec/2_model_old.tex <==
\section{Our Method: \model}
\label{sec:model}

As illustrated in Figure~\ref{fig:model}, \model~comprises 4 primary components:
(1) a mask proposal network that encodes the image into per-entity-level mask features;
(2) a mask decoder that decodes the mask features into pixel-level binary segmentation masks;
(3) an alignment network that transforms the raw mask features into visual tokens;
(4) an LLM that jointly processes the visual and text tokens.

The core design of \model is to formulate grounding as an \textit{entity selection} problem, with a pre-trained segmentation model to provide segmentation mask proposals for all the entities in the image. The feature associated with each mask proposal will be used as the visual input of the language model. Intuitively, this provides a structured entity-level understanding of the image, which naturally provides a good basis to perform grounding. Next, we will first introduce the mask proposal model and how it connects to the large language model (\S\ref{subsec:propose}). Then we illustrate how to use the representation produced by LLM to score mask proposals and retrieve the grounding mask (\S\ref{subsec:grounding}). Finally, we will show how our model architecture can naturally extend to support multi-modal user input, such as pointers that refer to a specific region in the image (\S\ref{subsec:pointer}). 

\subsection{Entity Mask Proposals}
\label{subsec:propose}

The mask proposal network module serves a dual purpose: providing pixel-level visual features for the LLMs and offering mask proposals that the LLMs can retrieve for language grounding.
We adopt a Mask2Former~\cite{cheng2022masked} as our mask proposal network for the visual encoder, which consists of an image encoder, a transformer query decoder, and a pixel decoder. 
The image is first encoded into continuous features through the encoder, which will be used in the pixel decoders to produce a set of multi-scale feature maps. 
The feature maps and a set of learnable queries are then fed to the transformer decoder, where the queries will progressively learn to capture the geometry and position of each entity through self-attention. 
The output queries from the final transformer layer will be used to decode the masks. 


In our experiment, we find that directly using the entity representations from Mask2Former leads to unsatisfied performance. 
Specifically, the model can distinguish simple objects by their categories, but fails to recognize simple concepts such as color. 
This is expected because the entity features are trained to produce accurate masks and recognize a limited number of object classes (133 classes predefined in COCO), where additional semantics about the entity's appearance are unnecessary and thus not learned. 
To address this issue, we leverage a CLIP~\cite{radford2021clip} model to provide the missing semantic information. 
In particular, we use the mask of each entity to extract the relevant CLIP patch features through a convolutional feature masking operator~\cite{dai2015convolutional}. 
To combine the pooled CLIP feature with the entity feature, we simply project the entity feature to the dimension of CLIP and sum them up.
The combined features are used as input for the language model. We use a two-layer MLP network to align the dimension between the visual features and input embeddings of the language model following \cite{liu2023improved}. 


\subsection{Grounding Language to Segmentation Masks}
\label{subsec:grounding}

The goal of language grounding is to connect text spans that refer to or can be deduced from visual information, known as \textit{groundable phrases}, to their corresponding visual elements~\cite{ma2023world}. Existing box-grounded vision-language models typically append location tokens after the groundable phrases~\cite{chen2021pix2seq,peng2023kosmos,chen2023shikra,you2023ferret}, which does not apply to our segmentation-based scenario. We thus introduce a pair of grounding tokens \texttt{<GRD>} and \texttt{</GRD>} to indicate the start and end of groundable phrases.
In Figure~\ref{fig:model-main}, a sentence can be represented as \texttt{I see <GRD> two dogs </GRD> on <GRD> the beach </GRD>}, with two distinct visual entities grounded. 
The representation of each groundable phrase is obtained by adding \texttt{<GRD>} and \texttt{</GRD>}'s output embedding from the last LLM transformer layer. 
The representation is then used to score each of the mask proposals on how likely it belongs to this groundable phrase. We find a simple linear head is enough to serve the purpose. Finally, we merge all the mask proposals into one single mask through the following pixel-wise maximization:
$$ \mathcal{M}_{h,w} = \max_q \left( \mathcal{S}_q \cdot \hat{\mathcal{M}}_{q,h,w} \right)$$
where $\mathcal{S}_q$ is the normalized score of the $q$-th mask between 0 and 1, and $\hat{\mathcal{M}}_{q,h,w}$ denotes the pixel probability at position $(h, w)$ for the $q$-th mask. Note that since the phrase may correspond to multiple entities, multiple mask proposals may get a high score at the same time and be picked jointly. One key advantage of \model~is that the selection of entities is fully transparent, and the user can easily see the visualize the mask proposals and the corresponding scores to understand how a grounding mask is predicted. 

\subsection{Pointer Input}
\label{subsec:pointer}

Attention and intention are natural in visually grounded dialogue, especially in reference resolution~\cite{malle2001intentions,prasov2008s}.
Several attempts and benchmarks have been proposed to expand the input space with additional pointers to spatial points, bounding boxes, and binary masks~\cite{zhu2016visual7w,mani2020point,you2023ferret}. 
We therefore introduce a pointer token \texttt{PTR} which refers to a specific point or region in the image input.
In Figure~\ref{fig:model-ptr}, a user instruction can be formed as \texttt{Describe the region <PTR> uniquely}, with requests the model for a referring expression about a specific region.
\texttt{PTR} serves as a placeholder token to be replaced by the visual token from the mask proposal, which corresponds to the actual pointer input.
Specifically, we compute the intersection-over-union (IoU) between the input pointer (either a box or a mask) to all mask proposals, and select the one with the best match.




==> vis/fig_teaser.tex <==
\makeatletter
\let\@oldmaketitle\@maketitle
    \renewcommand{\@maketitle}{\@oldmaketitle
    \vspace*{-20pt}
    \centering
    \includegraphics[width=1.0\textwidth]{figs/teaser_new.pdf}
    \vspace*{-20pt}
    \captionof{figure}{We propose \model, a multimodal large language model that enhances its text output with pixel-level phrase grounding across diverse semantic granularities. The figure demonstrates outputs from our model on the four task types we considered in this work.}
    \label{fig:demo}
    \vspace*{-5pt}
  \bigskip}
\makeatother

